Visually Dehallucinative Instruction Generation: Know What You Don't Know

"When did the emperor Napoleon invented iPhone?" Such hallucination-inducing question is well known challenge in generative language modeling. In this study, we present an innovative concept of visual hallucination, referred to as "I Know (IK)" hallucination, to address scenarios where "I Don't Know" is the desired response. To effectively tackle this issue, we propose the VQAv2-IDK benchmark, the subset of VQAv2 comprising unanswerable image-question pairs as determined by human annotators. Stepping further, we present the visually dehallucinative instruction generation method for IK hallucination and introduce the IDK-Instructions visual instruction database. Our experiments show that current methods struggle with IK hallucination. Yet, our approach effectively reduces these hallucinations, proving its versatility across different frameworks and datasets.

==> algorithm/prompt.tex <==
\begin{table}[H]
\caption{I Don't Know Aware Visual Instruction Generation Prompt}
\small
\begin{tabular}{p{1.0\linewidth}}
\toprule
\# I Don't Know Aware Visual Instruction Generation \\
\#\# Task Description\\
Carefully filtered VQA will be given, which is composed of a question and answers without an image and contains questions those are ambiguous to answer. The task is to generate proper answer. \\
\#\# Examples \\
\#\#\# VQA \\
Q: Is the bird female? \\
A: ['yes', 'yes', 'yes', "i don't know", 'no', 'yes', 'maybe', 'yes', 'yes', 'no'] \\
\#\#\# Answer \\
I don't know if the bird is female. It can be both male and female.  \\
\#\#\# VQA \\
Q: What word is on the ramp? \\
A: ['none', 'kcm', 'kcm', 'kcm', 'kck', 'kck', 'kcm', 'kck', 'kck', 'kek'] \\
\#\#\# Answer \\
I am not sure. It can be seen 'kcm', 'kck' or 'kek'. \\
\#\#\# VQA \\
Q: What gender is the person on the screen? \\
A: ['female', 'female', 'male', 'female', 'female', 'female', 'female', 'unknown', 'female', 'female'] \\
\#\#\# Answer \\
I am not sure the gender of the person on the screen. But it can be seen female. \\
\#\#\# VQA \\ 
Q: Where is the flash drive? \\
A: ["i don't see flash drive", 'in usb port', 'table', 'inserted in computer', 'on monitor stand', 'plugged into computer', 'no flash drive', 'none', 'computer', 'attached to computer'] \\
\#\#\# Answer \\
There is no flash drive in the image. However, it can be plugged into computer. \\
\#\#\# VQA \\ 
Q: What color is the disc? \\
A: ['silver', 'white', 'silver', 'no disc', "don't know", 'white', 'silver', 'silver', 'impossible', 'n'] \\
\#\#\# Answer \\
There is no disc in the image. \\
\#\#\# VQA \\
Q: How old is the dog? \\
A: ['5', 'unknown', 'young', '2', '1', '5', '2', 'middle age', '4', '3'] \\
\#\#\# Answer \\
It is unanswerable how old is the dog. \\
\#\#\# VQA \\
Q: Where is the water tank for the toilet located? \\
A: ['not pictured', 'bottom', 'no', 'unknown', 'behind toilet', 'not there', 'behind wall', 'underneath toilet', 'below', 'behind wall'] \\
\#\#\# Answer \\
It is unknown where the water tank for the toilet is located. It is not pictured. \\
\#\#\# VQA \\
Q: Is this person left or right handed? \\
A: ['left', 'right', 'left', 'right', 'unanswerable', 'left handed', 'left', 'left', 'right', 'left'] \\
\#\#\# Answer \\
It is unanswerable the person is left or right handed. \\
\#\# TASK \\
\#\#\# VQA \\
Q: \{question\} \\
A: \{answer\} \\
\#\#\# Answer \\
\bottomrule
\end{tabular}
\end{table}

==> figures/figidk.tex <==
\begin{figure}[!h]
\centering
\begin{minipage}[]{0.9\linewidth}
  \centering
  \centerline{\includegraphics[width=1.0\linewidth]{figures/idk1.png}}
%  \vspace{2.0cm}
  \centerline{(a)}\medskip
\end{minipage}
%
\begin{minipage}[]{0.9\linewidth}
  \centering
  \centerline{\includegraphics[width=1.0\linewidth]{figures/idk2.png}}
%  \vspace{1.5cm}
  \centerline{(b)}\medskip
\end{minipage}
%
\caption{
VQAv2 samples with the generated \idkb answer. 
}
\label{fig:idk}
\vspace{-0.3cm}
%
\end{figure}

==> figures/figmain.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=1.0\linewidth]{figures2/main.png}
\caption{
The proposed IDK visual hallucination categories and examples. 
}
\label{fig:main}
\end{figure*}

==> figures/figqual.tex <==
\begin{figure*}[htb]
  \centering
  \begin{minipage}{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/qual1.png}
    \label{fig:qual1}
  \end{minipage}
  \hfill
  \begin{minipage}{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/qual2.png}
    \label{fig:qual2}
  \end{minipage}

  \medskip

  \begin{minipage}{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/qual3.png}
    \label{fig:qual3}
  \end{minipage}
  \hfill
  \begin{minipage}{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/qual4.png}
    \label{fig:qual4}
  \end{minipage}
    \caption{Qualitative results.}
\end{figure*}

==> figures2/figlimit.tex <==
\begin{figure}[t]
\begin{tabular}{p{1cm}p{6cm}}
\toprule
& \includegraphics[width=\linewidth]{figures2/limitation.png} \\
User & What breed of horse is this? \\
\textbf{\textit{Ours}} & I don't know what breed the horse is. It could be a 'thoroughbred', 'quarter horse', 'mare', 'arabian', 'appaloosa', or 'standard’. \\
User & What health benefit does this type of vegetable have? \\
\textit{GPT4V} & I am sorry, but I cannot provide assistance in identifying or making assumptions about breeds of horses based on images. However, I can tell you that there are many breeds with various coat colors, body types, and characteristics. If you are interested in identifying horse breeds, you could consider factors such as the shape of the horse’s body, head, and ears, the texture of its coat, and the presence of any distinctive markings, and compare these with breed standards. Horse enthusiasts often consult with breed experts or use breed registries for accurate identifications. \\
\textit{Gemini} & The breed of this horse is a Criollo. \\
\textit{LLaVA} & The horse in the image is a Quarter Horse. \\
\bottomrule
\end{tabular}
\caption{Qualitative results on visual recognition and knowledge-requiring tasks.}
\label{fig:limit}
\end{figure}

==> figures2/figqualapp.tex <==
\begin{table*}[htb]
\caption{Qualitative results on IDK tasks. Underlines indicate the desired answer. Red
colored text indicates responses with visual hallucination.}
\begin{minipage}[t]{0.5\textwidth}
\vspace{0pt}
\begin{tabular}{p{1cm}p{6.5cm}}
    \toprule
    & \includegraphics[width=\linewidth]{figures2/qual3.png} \\
    User & What fruit is by the sink? \\
    \\
    \textbf{\textit{Ours}} & \underline{I am not sure.} It can be a banana or a banana bunch. However, there might be no fruit by the sink. \\
    \\
    \textit{GPT4V} & In the image provided, there isn't a clear view of the area by the sink, hence \underline{I cannot confirm} if there is fruit by the sink or identify any items in that specific area. The angle of the photograph focuses more on the refrigerator and the cabinet areas, not the sink or its surroundings. If you have an image that better captures the area near the sink, I'll be happy to assist you with that. \\
    \\
    \textit{Gemini} & \textcolor{red}{There is no fruit by the sink.} \\
    \\
    \textit{LLaVA} & \textcolor{red}{There is a banana by the sink.} \\
    \bottomrule
\end{tabular}
\end{minipage}%
\begin{minipage}[t]{0.5\textwidth}
\vspace{0pt}
\begin{tabular}{p{1cm}p{6.5cm}}
    \toprule
    & \includegraphics[width=\linewidth]{figures2/qual2.png} \\
    User & Is the elephant hot? \\
    \\
    \textbf{\textit{Ours}} & \underline{I don't know} if the elephant is hot. It can be both yes and no. \\
    \\
    \textit{GPT4V} & \underline{I cannot determine} the current temperature or how the elephant is feeling based on the image alone. Elephants are large animals that have various ways to regulate their body temperature such as flapping their ears, seeking shade, or taking a bath in water or mud. If it were a hot day, these behaviors could be indicative of the elephant trying to cool down. However, without more information or context, it's not possible to accurately state whether the elephant is hot. \\
    \\
    \textit{Gemini} & \textcolor{red}{The elephant is likely hot.} It is standing in the sun \textcolor{red}{with its ears spread out.} This is a common way for elephants to cool down. \\
    \\
    \textit{LLaVA} & \textcolor{red}{Yes, the elephant is hot, as it is standing in the shade and trying to cool off by drinking water.} \\
    \rule{0pt}{33.3ex} \\
    \bottomrule
\end{tabular}
\end{minipage}
\end{table*}
